Light Source Estimation with Analytical Path-tracing

We present a novel algorithm for light source estimation in scenes reconstructed with a RGB-D camera based on an analytically-derived formulation of path-tracing. Our algorithm traces the reconstructed scene with a custom path-tracer and computes the analytical derivatives of the light transport equation from principles in optics. These derivatives are then used to perform gradient descent, minimizing the photometric error between one or more captured reference images and renders of our current lighting estimation using an environment map parameterization for light sources. We show that our approach of modeling all light sources as points at infinity approximates lights located near the scene with surprising accuracy. Due to the analytical formulation of derivatives, optimization to the solution is considerably accelerated. We verify our algorithm using both real and synthetic data.

==> figures/ring_error.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
xmin=2,
xmax=28,
xtick={ 3,  5,  7,  9, 11, 13, 15, 17, 19, 21, 23, 25, 27},
xlabel style={font=\bfseries},
xlabel={Light Rings},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
ymin=0,
ymax=60,
ylabel style={font=\bfseries},
ylabel={Photometric Error},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left,align=left,draw=black}
]
\tiny
\addplot [color=white!60!blue,solid,line width=1.0pt,forget plot]
 plot [error bars/.cd, y dir = both, y explicit]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
3	28.8120419354839	1.32385798427027	1.32385798427027\\
5	13.1561125806452	3.51954026606693	3.51954026606693\\
7	10.0132696774194	2.13539870380605	2.13539870380605\\
9	8.16022935483871	1.89663104253118	1.89663104253118\\
11	9.62119419354839	1.90739492573296	1.90739492573296\\
13	11.6458170967742	2.79800259673479	2.79800259673479\\
15	10.89487	1.43675885483032	1.43675885483032\\
17	10.8305593103448	1.08458454257488	1.08458454257488\\
19	11.305975862069	2.89230446187134	2.89230446187134\\
21	10.3737728571429	1.11812246793902	1.11812246793902\\
23	11.5597928571429	3.25565771807225	3.25565771807225\\
25	12.1612137931035	3.60101772409394	3.60101772409394\\
27	11.6720079310345	3.05896745451839	3.05896745451839\\
};
\addplot [color=black!25!blue,solid,line width=1.0pt,mark size=1.7pt,mark=*,mark options={solid}]
  table[row sep=crcr]{%
3	28.8120419354839\\
5	13.1561125806452\\
7	10.0132696774194\\
9	8.16022935483871\\
11	9.62119419354839\\
13	11.6458170967742\\
15	10.89487\\
17	10.8305593103448\\
19	11.305975862069\\
21	10.3737728571429\\
23	11.5597928571429\\
25	12.1612137931035\\
27	11.6720079310345\\
};
\addlegendentry{One-light scenes};

\addplot [color=white!60!red,solid,line width=1.0pt,forget plot]
 plot [error bars/.cd, y dir = both, y explicit]
 table[row sep=crcr, y error plus index=2, y error minus index=3]{%
3	51.3520833333333	5.06835915126153	5.06835915126153\\
5	24.2905666666667	8.29990463963646	8.29990463963646\\
7	13.3892688888889	2.15847535178092	2.15847535178092\\
9	11.95457	3.22213846295757	3.22213846295757\\
11	13.54728	3.21806578185973	3.21806578185973\\
13	19.6623666666667	7.78959715351941	7.78959715351941\\
15	17.2791	3.88027323931765	3.88027323931765\\
17	16.8891588235294	2.26069304751298	2.26069304751298\\
19	18.4949117647059	3.27720845154118	3.27720845154118\\
21	17.45651875	4.12165903040976	4.12165903040976\\
23	19.6229	8.28664817603193	8.28664817603193\\
25	18.29539375	3.18795395794204	3.18795395794204\\
27	20.15345625	9.49487425431699	9.49487425431699\\
};
\addplot [color=black!25!red,solid,line width=1.0pt,mark size=1.7pt,mark=*,mark options={solid}]
  table[row sep=crcr]{%
3	51.3520833333333\\
5	24.2905666666667\\
7	13.3892688888889\\
9	11.95457\\
11	13.54728\\
13	19.6623666666667\\
15	17.2791\\
17	16.8891588235294\\
19	18.4949117647059\\
21	17.45651875\\
23	19.6229\\
25	18.29539375\\
27	20.15345625\\
};
\addlegendentry{Two-light scenes};
\addplot [color=black!25!yellow,solid,line width=1.0pt,mark size=1.7pt,mark=*,mark options={solid}]
  table[row sep=crcr]{%
3	53.3520833333333\\
5	26.2905666666667\\
7	15.3892688888889\\
9	13.95457\\
11	15.54728\\
13	21.6623666666667\\
15	19.2791\\
17	18.8891588235294\\
19	20.4949117647059\\
21	19.45651875\\
23	21.6229\\
25	20.29539375\\
27	22.15345625\\
};
\addlegendentry{Three-light scenes};

\end{axis}
\end{tikzpicture}%

